Self-Supervised Vision Transformers for Malware Detection

Malware detection plays a crucial role in cyber-security with the increase in malware growth and advancements in cyber-attacks. Previously unseen malware which is not determined by security vendors are often used in these attacks and it is becoming inevitable to find a solution that can self-learn from unlabeled sample data. This paper presents SHERLOCK, a self-supervision based deep learning model to detect malware based on the Vision Transformer (ViT) architecture. SHERLOCK is a novel malware detection method which learns unique features to differentiate malware from benign programs with the use of image-based binary representation. Experimental results using 1.2 million Android applications across a hierarchy of 47 types and 696 families, shows that self-supervised learning can achieve an accuracy of 97% for the binary classification of malware which is higher than existing state-of-the-art techniques. Our proposed model is also able to outperform state-of-the-art techniques for multi-class malware classification of types and family with macro-F1 score of .497 and .491 respectively.

==> tables/results-family.tex <==
\begin{table}[ht]
\centering
\caption{Results on malware family classification against 3 popular architectures ResNet, DenseNet and MobileNetV2—on macro-F1, macro-precision, and macro-recall.}

% \footnotesize
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lccc}
\hline
\textbf{Model}  & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} \\
\hline
% ViT-B(\sherlock) & .798 & .452 & .536 & .428  \\
% ViT-B (\sherlock) & .802 & .491 & .568 & .461  \\
ViT-B (\sherlock) & .491 & .568 & .461  \\
%0.5681352956809109, 0.46144056291695884, 0.4906652991449954
ResNet18 & .454 & .538 & .423 \\
ResNet50 &  .468 & .541 & .443 \\
DensetNet121 &  .461 & .529 & .438  \\
DenseNet169 & .462 & .545 & .434\\ 
MobileNetV2(x.5) &  .451 & .528 & .423 \\
MobileNetV2(x1) & .438 & .532 & .405 \\
\hline

\end{tabular}%
}
\label{table:results-family}
% \vspace*{-0.3in}
\end{table}





==> tables/results-type.tex <==
\begin{table}[ht]
\centering
\caption{Results on malware type classification against 3 popular architectures ResNet, DenseNet and MobileNetV2—on its accuracy, macro-F1, macro-precision, and macro-recall.}

% \footnotesize
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lrrccc}
\hline
\textbf{Model}  & \textbf{Accuracy} & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} \\
\hline
\sherlock & .836 & .418 & .609 & .374  \\
\sherlock V2 & .837 & .497 & .628 & .447  \\
%(0.6279113218062121, 0.4472304442859168, 0.49716807877257707
ResNet18 & - & .467 & .556 & .424\\
ResNet50 & - & .479 & .566 & .441\\
DensetNet121 & -& .471 & .558 & .428 \\
DenseNet169 & - & .477 & .573 & .433\\ 
MobileNetV2(x.5) & - & .460 & .547 & .424\\
MobileNetV2(x1) & - & .452 & .527 & .419\\
\hline

\end{tabular}%
}
\label{table:results-family}
% \vspace*{-0.3in}
\end{table}



